OSmosis: No more D\'ej\`a vu in OS isolation

Operating systems provide an abstraction layer between the hardware and higher-level software. Many abstractions, such as threads, processes, containers, and virtual machines, are mechanisms to provide isolation. New application scenarios frequently introduce new isolation mechanisms. Implementing each isolation mechanism as an independent abstraction makes it difficult to reason about the state and resources shared among different tasks, leading to security vulnerabilities and performance interference. We present OSmosis, an isolation model that expresses the precise level of resource sharing, a framework in which to implement isolation mechanisms based on the model, and an implementation of the framework on seL4. The OSmosis model lets the user determine the degree of isolation guarantee that they need from the system. This determination empowers developers to make informed decisions about isolation and performance trade-offs, and the framework enables them to create mechanisms with the desired degree of isolation.

==> Makefile <==
###############################################################################
# Configuration
###############################################################################

# The paper name without pdf extension
PAPER=main

# Build directory for the paper
BUILD_DIR=build

# the plots used in the apper
PLOTS=

# the figures that are used in the paper
FIGURES=

# optional build dependencies
DEPS_OPT=

# LATEXMK Options
LATEXMK_OPTS=\
	-latexoption=-interaction=nonstopmode \
	-output-directory=$(BUILD_DIR)

###############################################################################
# The paper targets
###############################################################################

FAIRYTALE=fairytale
FAIRYTALE_MAIN=fairytale-main.tex
FAIRYTALE_PDF=$(BUILD_DIR)/$(FAIRYTALE).pdf

PAPER_DRAFT=$(PAPER)-draft
PAPER_DRAFT_MAIN=main-draft.tex
PAPER_DRAFT_PDF=$(BUILD_DIR)/$(PAPER_DRAFT).pdf

PAPER_SUBMISSION=$(PAPER)-submission
PAPER_SUBMISSION_MAIN=main-submission.tex
PAPER_SUBMISSION_PDF=$(BUILD_DIR)/$(PAPER_SUBMISSION).pdf


PAPER_CAMREADY=$(PAPER)-camready
PAPER_CAMREADY_MAIN=main.tex
PAPER_CAMREADY_PDF=$(BUILD_DIR)/$(PAPER_CAMREADY).pdf

DEFAULT_MODE=$(PAPER_DRAFT_PDF)


###############################################################################
# Latexmk command definition
###############################################################################

# the latexmk command
LATEXMK=latexmk -pdf -logfilewarnings -f- $(LATEXMK_OPTS)


###############################################################################
# Dependencies
###############################################################################

DEPS_TEX=$(wildcard content/*.tex)
DEPS_BIB=$(wildcard content/*.bib)
DEPS_FIG=$(wildcard figures/**)
DEPS_PLOT=$(wildcard plots/**)

DEPS=Makefile $(DEPS_TEX) $(DEPS_BIB) $(DEPS_FIG) $(DEPS_PLOT) $(DEPS_OPT)


###############################################################################
# Make Targets (Building)
###############################################################################


default: $(DEFAULT_MODE)

all:  $(PAPER_DRAFT_PDF)  $(PAPER_SUBMISSION_PDF)

clean:
	rm -rf $(BUILD_DIR)/*

distclean: clean

$(FAIRYTALE_PDF) : $(DEPS) $(FAIRYTALE_MAIN)
	$(LATEXMK) -jobname="$(FAIRYTALE)" $(FAIRYTALE_MAIN)
	cp $(FAIRYTALE_PDF) $(BUILD_DIR)/$(FAIRYTALE)-latest.pdf
	@echo ""
	@echo "Built fairytale:    $(FAIRYTALE_PDF)"
	@echo "Updated latest: $(BUILD_DIR)/$(FAIRYTALE)-latest.pdf"

fairytale: $(FAIRYTALE_PDF)

$(PAPER_DRAFT_PDF) : $(DEPS) $(PAPER_DRAFT_MAIN)
	$(LATEXMK) -jobname="$(PAPER_DRAFT)" $(PAPER_DRAFT_MAIN)
	cp $(PAPER_DRAFT_PDF) $(BUILD_DIR)/$(PAPER)-latest.pdf
	@echo ""
	@echo "Built paper:    $(PAPER_DRAFT_PDF)"
	@echo "Updated latest: $(BUILD_DIR)/$(PAPER)-latest.pdf"

draft: $(PAPER_DRAFT_PDF)

$(PAPER_SUBMISSION_PDF) : $(DEPS) $(PAPER_SUBMISSION_MAIN)
	$(LATEXMK) -jobname="$(PAPER_SUBMISSION)" $(PAPER_SUBMISSION_MAIN)
	cp $(PAPER_SUBMISSION_PDF) $(BUILD_DIR)/$(PAPER)-latest.pdf
	@echo ""
	@echo "Built paper:    $(PAPER_SUBMISSION_PDF)"
	@echo "Updated latest: $(BUILD_DIR)/$(PAPER)-latest.pdf"

submission: $(PAPER_SUBMISSION_PDF)

$(PAPER_CAMREADY_PDF) : $(DEPS) $(PAPER_CAMREADY_MAIN)
	$(LATEXMK) -jobname="$(PAPER_CAMREADY)" $(PAPER_CAMREADY_MAIN)
	cp $(PAPER_CAMREADY_PDF) $(BUILD_DIR)/$(PAPER)-latest.pdf
	@echo ""
	@echo "Built paper:    $(PAPER_CAMREADY_PDF)"
	@echo "Updated latest: $(BUILD_DIR)/$(PAPER)-latest.pdf"

camready: $(PAPER_CAMREADY_PDF)


.PHONY: all clean rebuild-figures $(PAPER_DRAFT_PDF) $(PAPER_SUBMISSION_PDF) $(PAPER_CAMREADY_PDF)


figures/%.pdf: figures/%.svg
	inkscape $< --export-area-drawing --export-pdf=$@


###############################################################################
# Make Targets (Open)
###############################################################################

view-draft: $(PAPER_DRAFT_PDF)
	xdg-open $(PAPER_DRAFT_PDF)

view-submission: $(PAPER_SUBMISSION_PDF)
	xdg-open $(PAPER_SUBMISSION_PDF)

view-camready: $(PAPER_CAMREADY_PDF)
	xdg-open $(PAPER_CAMREADY_PDF)

view-latest:
	xdg-open $(BUILD_DIR)/$(PAPER)-latest.pdf


==> content/allocator_notes.tex <==
% !TEX root = ../main-draft.tex
\section{Allocator notes}

I was thinking something like this.

Say, `R\_T1` is a resource of type `T1` And an allocator 
is initialized with `R\_T1` and hands out resources of either type `R\_T1` or type `R\_T2`.

In either case, it needs to keep the mapping information in a table of sort sorts e.g., page-table, inode blocks on disk, etc.

Let's say the PD wants an extra degree of isolation for the allocator that does `R\_T1---->R\_T2`.
Then we have two options:
\paragraph*{Option 1}

This setup: We take 2 allocations `R\_T2` from `A1`, and then create two allocators.  
This is running two FS on the same block driver. Or like the virtual memory systems
 when Virtual Machines i.e. nested translations. `R\_T2\^` is of the same type as R\_T2, but in a
 different namespace. 
 Like in the case of nested virtual memory, you again get the entire 2\^64 space, 
 but in the case of malloc, you only get a sub range.

\begin{verbatim}
R\_T1  --A1--> R\_T2 --- A\_after---> R\_T2^
                \
                 \-----A\_after---> R\_T2^
\end{verbatim}
or

\paragraph*{Option 2}
This setup: We take R\_T1 before A1 and then create two allocators which return sub-regions of R\_T1(either disjoint ranges or time shared).  This is like two driver stacks on an existing driver (sort of like Virtual Machines do)

\begin{verbatim}
2. R\_T1 ----A\_before---> R\_T1 --A1--> R\_T2 
      \
       \----A\_before---> R\_T1 --A1--> R\_T2 

\end{verbatim}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[h!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|}
\hline
No & Input Type & Output Type    & New namespace      & Time Sharing Underlying resourse & Eg                                                             \\ \hline
1 & R\_T1 & R\_T1 & No & No & malloc \\ \hline
2  & R\_T1      & R\_T1          & Yes (using offset) & Not sure.                        & PID namesapce(no time sharing), chroot                         \\ \hline
3 & ?     & ?     & ?  & ?  & ?      \\ \hline
4  & R\_T1      & \textbf{R\_T2} & NA                 & Yes                              & Disk to File and most other things. Virtual to physical memory \\ \hline
\end{tabular}%
}
\caption{}
\label{tab:my-table}
\end{table*}


I think as soon as we introduce the time division multiplexing of a resource, we should consider it a new resource.

Why did I make this table? I am trying to capture all types of allocators
\begin{verbatim}
- namespaces
- Virtual memory
- Drivers
- File systems
- NW Stacks
- Schedulers 
\end{verbatim}

When it comes to the mapping inside an allocator, we can say that there are two ways of doing that

\begin{verbatim}
- HW assisted.
- Purely SW.
\end{verbatim}

And I think that is a neat wrap.

==> content/formalization.tex <==
% !TEX root = ../main-draft.tex

\section{Model Formalization}

\RA{An attempt to formalize the model}

\subsection{Model}

We first define the core the isolation model.
Users of a system care about their objects: that is either some malloced() piece of memory, a file, a thread, EP-to query system state etc.
%
\begin{align*}
    \textit{Object} &= \textit{Something of interest for the user (malloc, file, thread)}
\end{align*}
%
Those objects live or reside in the resources of the system.

\SA{ Talk about permissions.}

\SA{Objects can also be comm-endpoints (syscalls) to the kernelstate/driver/FS/VM-system,
Things like, how much space is remaining etc.
}
%
Users may not necessarily care where those objects live as long as they can access them.
%
For example, a user cares about getting back the file contents, but doesn't care where on disk the file is stored.
\RA{Maybe talk about resource slices here?}
\begin{align*}
    \textit{Resource} &= \textit{RAM, Blocks, Kernel State, ...}
\end{align*}
%
Objects are allocated within a given resource.
%
That might be a partition on disk, a chunk of virtual memory backing the heap or alike.
%
Thus, we have the concept of an allocator that will allocate new object from an underlying resource.
%
\RA{do we need designated resources from which can be allocated? See \textit{ResourceLocations} relation below.}
%
\begin{align*}
    \textit{Allocator<Resource>} &= \textit{Allocate objects from a resource}
\end{align*}
%
The protection domain is the a set of objects the user has allocated and a set of allocators the
user can allocate new objects from.
%
Thus, the set of allocators define the set of resources from which the protection domain may allocate.
%
\RA{Can the protection domain be granted access to objects without having an allocator? }
%
\begin{align*}
    \textit{PD} &= (\textit{Set<Objects>}, \textit{Set<Allocator>})
\end{align*}
%
The system may create copies of the objects in different other resources.
%
For example, the CPU cache contains a copy of DRAM contents, or the page cache contains a copy of
the contents on disk.
%
Thus, we have a  relation that captures where the system may place parts of other resources by
associating resources with other resources.
%
\begin{align*}
    \textit{ResourceLocations} &:: \textit{Resource} \times  \textit{Resource}
\end{align*}
%

Finally, we can define the system as a set of protection domains and a set of resources.
\begin{align*}
    \textit{System} &= (\textit{Set<PD>}, \textit{Set<Resources>})
\end{align*}

This defines our isolation model.



\RA{Maybe have the "System" that is a set of PDs and a set of Resources or allocators?}.

\subsection{Queries}

Based on the model, we can now define queries and predicates on the model to specify the level of
isolation.

The \textit{ResourceLocations} relation lists the possible ``one-hop'' locations of a resource.
%
To obtain \emph{all} possible locations, we take the reflexive transitive closure of the relation.

\begin{align*}
    \textit{AllResourceLocations} & :: \textit{Resource}\Rightarrow  \textit{Set<Resource>}\\
    \textit{AllResourceLocations} & :: r = ResourceLocations^*(r)
\end{align*}
%
Because every object has been allocated from a specific resource, we can define the \textit{ResourceOfObject}
function that obtains the resource from which an object has been allocated.
%
\begin{align*}
    \textit{ResourceOfObject} & :: \textit{Object}\Rightarrow  \textit{Resource}
\end{align*}
%
\RA{Maybe this relation should be part of the model, as this may change, see time shared)}
%
Using the \textit{ResourceOfObject} function we can now define the \textit{ResourcesOfPD} function that
lists all the resources the protection domain currently has access to.
%
\begin{align*}
    \textit{ActualResourcesOfPD} & :: \textit{PD}\Rightarrow  \textit{Set<Resources>}\\
    \textit{ActualResourcesOfPD} & :: pd = \bigcup_{o \in Objects} \textit{ResourceOfObject}~o\\
\end{align*}
%
With the functions above we can now define the function \textit{ResourcesOfPD} that lists all
resources that the protection domain may have access to. This is the union of all resources the
allocated objects may reside in and all resources the protection domain may allocate from.
%
\begin{align*}
    \textit{ResourcesOfPD} & :: \textit{PD}\Rightarrow  \textit{Set<Resources>}\\
    \textit{ResourcesOfPD} & :: pd =
                           \bigcup_{r \in ActualResourcesOfPD pd }  \textit{AllResourceLocations}~r \\
                           & \cup
                           \bigcup_{r \in AllocatorResources pd }  \textit{AllResourceLocations}~r \\
                           & \cup \delta
\end{align*}
Where, $\delta$ are the unknown resources or the resources we don't quite care about with regards
to isolation.
\RA{this is meant to express some unknown state that is not captured in the model}


\subsection{Stating Isolation Levels}

\paragraph{Weak Isolation}
Two protection domains share access to an object, if they have the object within their own set of
objects.
%
Hence, the shared objects between two protection domains is the intersection of their sets of objects.
%
\begin{align*}
    \textit{SharedObjects} & :: \textit{PD} \Rightarrow \textit{PD}\Rightarrow  \textit{Set<Object>}\\
    \textit{SharedObjects} & :: pd_1~pd_2 = pd_1.0 \cap pd_2.0
\end{align*}
%
\RA{the .0 here means the first element of the tuple, which is the set of objects}
%
We say, two protection domains are \emph{weak isolated} if they do not share any objects.
\begin{align*}
    \textit{WeakIsolated} & :: \textit{PD} \Rightarrow \textit{PD}\Rightarrow  bool\\
    \textit{WeakIsolated} & :: pd_1~pd_2 \Leftrightarrow \textit{SharedObjects}~ pd_1~pd_2 = \emptyset
\end{align*}
%
Shared libraries and kernel state aside, two processes can be considered \emph{weak isolated}.

\SA{Even in case of weak isolation, there might be many objects that are shared, eg, processes share the same syscall interface.
We can express that as a -$\delta$ or some other symbol to signify intentional ignoring of common things.}

\paragraph{Strong Isolation}
Similarly, two protection domains may not have accecss to the same objects and thus are weak isolated,
but still they share access to some of the underlying resources.
%
We define the set of shared resources between two protection domains as the intersection of the
resources they have access to.
%
\begin{align*}
    \textit{SharedResources} & :: \textit{PD} \Rightarrow \textit{PD}\Rightarrow  \textit{Set<Resource>}\\
    \textit{SharedResources} & :: pd_1~pd_2 = \textit{ResourcesOfPD}~pd_1 \cap \textit{ResourcesOfPD}~pd_2
\end{align*}
%
We say that two protection domains are \emph{strong isolated} if they do not share any of the underlying
resources. This includes \emph{all possible} resources the protection domain may have access to.
%
\begin{align*}
    \textit{StrongIsolated} & :: \textit{PD} \Rightarrow \textit{PD}\Rightarrow  bool\\
    \textit{StrongIsolated} & :: pd_1~pd_2 \Leftrightarrow \textit{SharedResources}~ pd_1~pd_2 - \delta = \emptyset
\end{align*}
%
Note, we subtract $\delta$ to exclude unknown resources that are part of both protection domains.
%
Thus we can precisely state that two protection domains are \emph{strong isolated} with respect to
the set of unknown resources $\delta$. Moreover, $\delta$ may also include resources we don't care
about with regards to isolation.

\paragraph{Relaxed Isolation}
We can relax the notion of strong isolation by just taking the actual resources the protection domain
has access to into account, and not all possible locations.
%
\begin{align*}
    \textit{SharedResources}' & :: \textit{PD} \Rightarrow \textit{PD}\Rightarrow  \textit{Set<Resource>}\\
    \textit{SharedResources}' & :: pd_1~pd_2 = \textit{ActualResourcesOfPD}~pd_1 \cap \textit{ActualResourcesOfPD}~pd_2
\end{align*}
%
\RA{probably have a better name..}
%
And we define the \textit{RelaxedIsolated} as the $\textit{SharedResources}'$ being empty. Note,
given the actual resources of a protection domain only includes known resources, we do not need
to subtract $\delta$ here.
%
\begin{align*}
    \textit{RelaxedIsolated} & :: \textit{PD} \Rightarrow \textit{PD}\Rightarrow  bool\\
    \textit{RelaxedIsolated} & :: pd_1~pd_2 \Leftrightarrow \textit{SharedResources}'~ pd_1~pd_2 = \emptyset
\end{align*}

\paragraph{PD Isolation}

\begin{align*}
    \textit{Isolated} & :: \textit{PD} \Rightarrow \textit{System} \Rightarrow IsoFn \Rightarrow  bool\\
    \textit{Isolated} & :: pd~sys = \forall pd' \in \textit{PDs}~sys. \textit{IsoFn}~pd~pd'.
\end{align*}


\subsection{Time Shared}
Time sharing is an important concept. The most prominent example there of are processors, but also
memory (swapping) and file systems (page cache) can be seen as some for of time shared access
to resources. There are two aspects there of:

\paragraph{Transparent Time Sharing} Where the user does not realize that the resource is shared. For
example, a thread is being descheduled: the thread context is copied from the CPU registers to
some other location, or a page is swapped out to disk. In both cases, this happens transparently to
the user. This often requires some for of virtualization.

In this case we do not necessarily need to do anything, as this is already expressed in the model
(i.e., all possible locations are expressed)
%
As seen from the user, the object is still at the same (virtualized) location.

\paragraph{Explicit Time Sharing}
In this case, the user explicitly move the object to a different location. For example, an application
storing some of its data on disk, e.g., a text editor saving the document before opening a new one.
In this case, the location of the object changes.

We can express this as a transition in the state of the model: protection domain allocates a new object
from one of its allocators and then copies the contents, and releasing the old object.

\subsection{Virtualization: Objects become resources?}

\RA{so this is just a thought for now}

Finally, we talk about the notion of different levels of nesting or virtualization. There are many
examples where this is already happening in real life: virtual machines virtualize CPUs and memory,
The object (vCPU) as seen from the host becomes a resource (CPU) as seen from the guest. Similarly,
physical memory assigned to the virtual machine (object) becomes guest physical memory (resource)
in the guest. Likewise, the swapfile (object) becomes a resource (memory) as seen from processes.

Thus as virtual machine monitor exposes objects on its level (memory, cpu,, devices, ...) to the
guest as resources.

We can say that a virtualized resource (\emph{vResource}) is a resource that is virtualized out
of a collection of objects.
\begin{align*}
    \textit{vResource} &= \{ Object \}
\end{align*}

\RA{not sure if we need to do this distinction here. We can simply have the transitive closure
of the resources relation. and distinguish the virtualized resources from the actual resources
using the "terminals" of the relation, i.e., resources that do not have an element in the relation
where they appear on the left hand side.
}

\section{Use Cases}

\paragraph*{Process}

What a Process would look like:
\begin{itemize}
    \item Object 
    \begin{itemize}
        \item VM: Stack, Heap, Code, Memory-mapped-file, \\shared-memory-region
        \item CPU: Thread-Control?
        \item Storage: CWD
        \item Networking: Sockets
        \item Misc: Ungatergorized RPC calls to change/know the system state
        % \item Syscall: Ability to do RPC to kernel/other services
    \end{itemize}
    
    \item Allocators:
    \begin{itemize}
        \item: Virtual Memory Allocator EP, 
        \item Physmem-Allocator-EP, 
        \item CPU-Allocator(to make new threads), 
        \item Phys-CPU-allocator
        \item File desc allocator
        \item Disk block allocator
        \item Socket allocator
        \item NIC allocator?
    \end{itemize}
    
    \item Resouces for each object:
    \begin{itemize}
        \item: stack/heap/code: pages, caches, regs, swap, uArch (write buffers, BTB, ... $\delta$) 
        \item: CPU: regs, uArch (write buffers, BTB, ... $\delta$), CPU-core, scheduler
        \item: Storage: file-system, open-file table, disk, caches, CPU
        \item: Network: NIC, NW stack(--> memory, and others ), 
        \item: RPC: The PD which answers to that PD
    \end{itemize}
\end{itemize}

To now express a process that does code-dedup, the code object between two processes

Process have their own virtual memory and have their virtual memory allocator, and also own heap and stack object.
However, they may share the code object.

They have their own thread control block, but might share the physical CPU allocator.

They share the global open file table, but share their own local file table, and can share the same memory mapped file.


Two processes are weakly isolated if do not share any objects, but even that is stronger than the normal process deinition in a Unix system.
As they share the states in the kernel(PID space, filesystem, ..), which shows up as objects in the PD.

Say two processes have, their own endpoints to talk to the file systems, the objects and allocators are not shared, so it would be weak isoalted.
Now we do the resolution step, the allocators are created/backed by objects(in another PD). This object might itself be allocated 
from the same allocator, which might be shared.

\begin{verbatim}
PD1: Object -> Allocator --< object
                                ^
                                |
                    PD-X:  allocator   
                                |
                                v
PD2: Ojbect -> Allocator --< object
/******************************/
    
PD1: Object -> Allocator --< object
                                ^
                                |
                    PD-X:  allocator  --< object
                                            ^
                                            |
                                  PD-Z:  allocator  
                                            |
                                            v
                    PD-Y:  allocator  --< object

                                |
                                v
PD2: Ojbect -> Allocator --< object
    
\end{verbatim}


But in some way it is not strongly isolated as the EP objects are contrcuted/backed by the 


\paragraph*{Thread}


\paragraph*{Thread With Isolated Stack}


\paragraph*{Light Weight Context}
\paragraph*{Container}
\paragraph*{Virtual Machine}

The GPA will be an allocator which is created by an object which is part of the VMM.
The VMM may allocate the physical memory.

Similarly, for the CPU, we create a vCPU object and this will become the CPU allocator of the VM.

\paragraph*{Unikernels}
On a first approximation, Unikernels are similar to virtual machines, but many of the allocators mentioned previously 
are either merged into the application i.e. they are in the same PD. Or are removed from the VM and replaced by a simplified layer.



==> content/framework_old.tex <==
% !TEX root = ../main-draft.tex
\section{\system Framework}
\label{sec:framework_old}

In this section, we describe the building blocks needed from
the system to realize the model.


% \subsection{Capabilities}

\subsection*{Protection Domain}
Just like in the model, the framework has the notion of the Protection Domain.
It is a collection of resources used to run a task.


\subsection*{Abstract Resource Manager}
An \emph{Abstract Resource Manager} maintains the \emph{associated state} of an \emph{abstract resouce}.
The \emph{Abstract Resouce Manager} in OSmosis is a wrapper around a subsystem(e.g., file system, networking stack)
in a typical OS.


\MIS{I worry about using an acronym ARM -- it's a processor to this community.}
\SA{Agreed, won't use the acronym}
Besides the APIs expected from a subsystem, subsystems wrapped in an \emph{abstract resource manager} give
us two additional functionalities.
1) It gives us a way to run two isolated instances of the subsystems.
\SA{For example, ...}
2) Provides an allocator for the underlying resource it is abstracting.
\SA{In the case of the file-system, it is an allocator to physical blocks,
and for virtual memory, it is physical memory.}

\SA{Do we need a abstract-resouce-manager or is an allocator the right abstraction?}

% Allocators are initialized with a resource of a lower level (\SA{or same level}),
% for eg., a virtual memory allocator is initiated with physical memory, but it can also
% be initialized with virtual memory itself (think two levels of translation in VMM).

% If two virtual memory allocators are initialized with a disjoint set of physical memory, then
% it is not possible to establish sharing between the allocated virtual memory ranges.
% Allocators operate on disjoint sets of resources and are the means to achieve physical isolation.

\subsection*{Resource Delegation and Permissions}
PDs have access to resources with specific permission.
It can delegate access to resources to other PDs as long
as the PDs also share the abstract resource manager for that resource.

\SA{
I think the following is an important discussion to be had, but not sure where.
Virtual-memory translates addresses with assistance from hardware.
Specifically, once the mapping of the \textbf{virtual memory (abstract resource)} to \textbf{physical memory(physical resource)}
is set, the software stays out of the way, i.e., no software check on every read/write.
In contrast, \texttt{chroot} translates paths, but the software is involved in every access(e.g., open)
}



% \subsection*{Allocator}


% \subsection*{Boundary Generator}
% Additional abstraction can be run in the same domain or not.
% In a microkernel, different subsystems are in a separate address space.
% However, in a monolithic kernel, they are in the same address space.
% FlexOS showed that these boundaries are can blurred,
% and subsystems can be combined based on the performance and isolation needed.
% Furthermore, in the contemporary hardware landscape,
% virtual memory and access control are beginning to decouple with features like
% Intel-MPK, ARM-MTE, and CHERI/Morello.


% \SA{
% There will be note at the end about how virtualizing CPU automatically
% raises the virtualizing the memory too.
% }

\subsection*{One API to rule them All?}
We present a \texttt{clone} \MIS{citation} \SA{ack} like API we call \texttt{make-a-thing}.
\MIS{Turn "make-a-thing" into a macro so we can come up with a new, something like
newPD might work -- make-a-thing was not intended to every be real.} \SA{ack}
\MIS{This next sentence isn't quite correct -- you have N things, each of which
has a resource type and a degree of sharing; you can make that types implied so
you pass just a single N-tuple; but you can't have a single tuple of only 2 things.} \SA{ack}
This API takes in a N-tuple, where the first element of
the tuple is the resource type, and the second element is the extent to which
that element is shared with its parent.

% For each of the resources and associated states,
% we pick how isolated it is from the parent.
% If a higher level of isolation is picked for the associated state,
% sharing a resource from that subsystem is not possible.
% For ex., if the filesystem state for two PD is completely isolated,
% they cannot share files(resources).

% \SA{Show the pseudo code here.}
% \input{algo/make-a-thing.tex}


==> content/implementation.tex <==
% !TEX root = ../main-draft.tex

\section{Implementation}
\label{sec:implementation}

\SA{Not sure if this section is adding value in \underline{this} paper.}

We have implemented a small portion of \system, which exposes memory objects, 
using the capabilities-based microkernel seL4~\cite{seL4Website}.
We chose a microkernel as it has no existing notion of a process, container, or virtual machine.
This lack of existing abstractions allows us to define the building blocks as we see fit.
\emph{Capabilities} and \emph{capability spaces} map well to
\system's resources and protection domains.
Capabilities are a natural fit for our framework as they facilitate the easy exchange of resources.
% \MIS{Will anyone understand what this setence means?}
% The capabilities in \system are at a higher level of granularity than seL4.



==> content/model_old.tex <==
% !TEX root = ../main-draft.tex
\section{\system Isolation Spectrum Model (old)}
\label{sec:model_old}

\begin{figure}[hb]
\centering
\includegraphics[width=0.7\columnwidth]{figures/model-mini.png}
\caption{Model \RA{there should not be an arrow from 4 to allocator, no?}
               \SA{I think yes, the PD has a DRAM allocator so that the VMem abstract-resource is backed by DRAM from that pool. 
                   It need not always have one, in which case some default one will be used by that associated state} 
}
\label{fig:model-mini}
\end{figure}

\SA{Each para has the following narrative
\begin{itemize}
    \item Introduce a new term/concept.
    \item Explain why we need it.
\end{itemize}
}



We view an OS isolation mechanism (e.g., process, containers, virtual machines)
as a collection of resources that we call a \emph{Protection Domain(PD)}.
Each PD is an \textbf{N-tuple},
where N is the number of different resources from which we assemble
the mechanism, and each element of the N-tuple indicates the
the degree to which the resource is shared.
\SA{Give examples of what resources can be}.
A resource can be either \emph{abstract} or \emph{physical}.

\RA{A thought: In some way PDs (applications, ...) care about their objects (e.g., memory, files, ...)
and maybe a bit less about the actual resources they use (e.g., virtual/physical memory, blocks on disk, ...)
in which resources (abstract of physical) those objects are stored is defined by the isolation mechanism
that defines the allocation of objects to resources. } \SA{I like this terminilogy.}

Every \emph{abstract} resource maps to another resource
with mapping information in \emph{associated state}.
\SA{Give concrete about the associated state, for instance, how containers share associated state}.

When discussing resource sharing, we have had to take into
account the sharing of the resource itself and its associated state.
\SA{When associated state is shared, we are exposed to a class of bugs.}

Resources can be shared in one of the four different configurations.
\begin{itemize}
    \item Shared
    \item Partially Shared
    \item Isolated
    \item Time Shared
\SA{We will introduce Objects here and thus shared Vs. Hidden Objects}
\end{itemize}

\MIS{I don't understand the following two items.}
\SA{This is odd}This lets us model the aspects of resources that can hold Objects
but are not yet known to us. \SA{The previous line should be removed and the content will be rolled into Time Shared.}

\RA{Could we say that an object viewd from one PD could be a resource viewd from another PD,
for example: your virtual disk image is a resource for your VM, but it is also an object for Qemu?}
\SA{Absolutely!}

Similar to resources, the associated state can also be shared or isolated.
\SA{Need to explain why that is.}
% \begin{itemize}
%     \item Shared
%     \item Partially Shared
%     \item Isolated
% \end{itemize}



\subsection*{Viewing Associated State as separate PD}
Associated states for different resources can be in the same PD or not.
\SA{For instance, in a monolithic OS the scheduler and filesystems both reside
in the kernel and a buffer over run bug in the filesystem can potentially crash the
scheduler. In contrast, in a microkernel they are in separate address spaces.}
Containers add a level of abstraction for certain abstract resources,
but that additional associated state is still in the same protection domain.



Visualizing the resource dependence as DAG, it becomes trivial to find out what is shared and isolated
between two PDs.
\MIS{This probably requires a picture so that the reader is seeing
what you are imagining they are seeing.} \SA{ack}
\SA{...
 Then start two \emph{Breadth First Searches} from the two PDs. ...
}
% \SA{There can be loops in our graph(which makes it not be a DAG), for instance VM subsystems
% used FS for swap, and swap systems uses VM subsystem for their own memory
% I(sid), need a way to decouple this cycle.

% }




\begin{figure*}[ht]
\centering
\includegraphics[width=1\textwidth]{figures/usecases.png}
\caption{Different mechanisms are seen under OSmosis}
\label{fig:model-main}
\end{figure*}

\subsection*{Putting it all together}
As an example to make this clear \autoref{fig:model-main} shows how increasing isolation of resources changes thread to a process and all
the way to a VM.
\SA{...}
Thus we see that different mechanisms are nothing more than a collection of resources with different levels of sharing for those resources
and their associated state.







% \subsection*{Identifying the extent of sharing}

% Both virtual resources and physical resources can be shared
% in one of the following configurations.

% \begin{itemize}
%     \item Completely shared
%     \item Partially shared
%     \item Time shared
%     \item Not at all shared (Completely Isolated)
% \end{itemize}

% Associated State can be similarly shared in the following configurations:

% \begin{itemize}
%     \item \SA{Not sure if it same as above.}
% \end{itemize}


==> content/relatedwork.tex <==
% !TEX root = ../main-draft.tex

\section{Related Work}
\label{sec:relatedwork}

\SA{A condensed version of the same section from the RPE report.}

\subsection{Specific Mechanisms}

\subsection{Frameworks}

